Successive-Cancellation Flip Decoding of Polar Codes Under Fixed Channel-Production Rate

Polar codes are a class of error-correcting codes that provably achieve the capacity of practical channels under the low-complexity successive-cancellation flip (SCF) decoding algorithm. However, the SCF decoding algorithm has a variable execution time with a high (worst-case) decoding latency. This characteristic poses a challenge to the design of receivers that have to operate at fixed data rates. In this work, we propose a multi-threshold mechanism that restrains the delay of a SCF decoder depending on the state of the buffer to avoid overflow. We show that the proposed mechanism provides better error-correction performance compared to a straightforward codeword-dropping mechanism at the cost of a small increase in complexity. In the region of interest for wireless communications, the proposed mechanism can prevent buffer overflow while operating with a fixed channel-production rate that is 1.125 times lower than the rate associated to a single decoding trial.

==> data/used_slots_dscf_100_cw_drop_2_25_9_8.tex <==
idx  slots
1  10
2  15
3  48
4  42
5  45
6  75
7  92
8  93
9  97
10  92
11  99
12  97
13  96
14  95
15  88
16  88
17  87
18  91
19  98
20  88
21  95
22  84
23  82
24  86
25  97
26  98
27  95
28  93
29  98
30  92
31  98
32  98
33  96
34  94
35  89
36  85
37  98
38  97
39  88
40  97
41  99
42  98
43  96
44  99
45  92
46  94
47  98
48  99
49  96
50  94
51  97
52  87
53  98
54  94
55  99
56  98
57  95
58  95
59  90
60  92
61  98
62  99
63  97
64  89
65  98
66  99
67  96
68  90
69  94
70  98
71  97
72  79
73  98
74  97
75  93
76  97
77  98
78  98
79  89
80  85
81  99
82  94
83  98
84  97
85  91
86  95
87  99
88  96
89  98
90  99
91  99
92  99
93  92
94  93
95  98
96  93
97  96
98  89
99  93
100  93
101  93
102  93
103  90
104  97
105  99
106  94
107  97
108  99
109  99
110  99
111  99
112  97
113  99
114  95
115  98
116  93
117  95
118  92
119  86
120  94
121  92
122  99
123  93
124  91
125  84
126  98
127  99
128  90
129  92
130  96
131  95
132  97
133  82
134  86
135  97
136  96
137  92
138  93
139  98
140  97
141  99
142  87
143  91
144  99
145  98
146  98
147  97
148  82
149  96
150  94
151  91
152  99
153  97
154  98
155  91
156  93
157  97
158  97
159  99
160  89
161  99
162  93
163  92
164  96
165  89
166  95
167  98
168  98
169  91
170  99
171  98
172  99
173  91
174  90
175  88
176  99
177  96
178  98
179  99
180  91
181  87
182  78
183  94
184  95
185  94
186  95
187  97
188  90
189  98
190  99
191  93
192  87
193  97
194  98
195  87
196  98
197  95
198  99
199  95
200  99
201  94
202  98
203  94
204  95
205  91
206  88
207  98
208  97
209  95
210  93
211  81
212  96
213  98
214  90
215  91
216  99
217  96
218  99
219  95
220  96
221  98
222  99
223  97
224  96
225  91
226  94
227  98
228  97
229  98
230  99
231  85
232  92
233  91
234  99
235  89
236  95
237  97
238  98
239  99
240  87
241  98
242  98
243  97
244  99
245  98
246  97
247  89
248  98
249  99
250  99
251  94
252  98
253  83
254  98
255  93
256  94
257  84
258  99
259  96
260  97
261  93
262  99
263  98
264  96
265  97
266  97
267  99
268  98
269  89
270  98
271  97
272  97
273  98
274  95
275  90
276  96
277  99
278  88
279  90
280  93
281  99
282  99
283  98
284  93
285  90
286  99
287  95
288  97
289  98
290  91
291  93
292  99
293  95
294  94
295  83
296  99
297  98
298  90
299  99
300  98
301  98
302  88
303  92
304  95
305  93
306  87
307  97
308  95
309  99
310  98
311  93
312  98
313  96
314  88
315  99
316  95
317  84
318  96
319  93
320  91
321  92
322  87
323  96
324  99
325  92
326  84
327  95
328  95
329  98
330  95
331  99
332  99
333  98
334  95
335  97
336  85
337  97
338  90
339  93
340  96
341  94
342  98
343  99
344  93
345  93
346  91
347  97
348  88
349  94
350  96
351  94
352  98
353  97
354  92
355  87
356  85
357  90
358  99
359  85
360  99
361  95
362  97
363  97
364  95
365  99
366  98
367  96
368  98
369  99
370  75
371  67
372  96
373  93
374  97
375  95
376  98
377  97
378  76
379  99
380  98
381  90
382  91
383  99
384  91
385  98
386  96
387  99
388  90
389  97
390  94
391  86
392  99
393  89
394  94
395  97
396  96
397  97
398  98
399  91
400  97
401  95
402  96
403  75
404  86
405  90
406  97
407  97
408  91
409  94
410  89
411  91
412  98
413  92
414  97
415  94
416  96
417  97
418  96
419  98
420  99
421  98
422  99
423  96
424  98
425  95
426  95
427  98
428  96
429  98
430  92
431  93
432  92
433  93
434  94
435  97
436  94
437  97
438  94
439  99
440  96
441  96
442  97
443  91
444  93
445  96
446  85
447  90
448  99
449  97
450  99
451  99
452  99
453  93
454  87
455  98
456  96
457  99
458  99
459  89
460  99
461  95
462  99
463  97
464  99
465  99
466  97
467  97
468  92
469  90
470  93
471  96
472  94
473  96
474  98
475  96
476  95
477  97
478  98
479  99
480  97
481  98
482  87
483  95
484  99
485  89
486  99
487  98
488  96
489  98
490  96
491  80
492  86
493  90
494  97
495  98
496  92
497  96
498  98
499  96
500  99
501  93
502  92
503  99
504  98
505  88
506  99
507  97
508  89
509  99
510  86
511  84
512  98
513  93
514  92
515  99
516  93
517  96
518  96
519  92
520  88
521  83
522  97
523  98
524  95
525  97
526  99
527  93
528  99
529  96
530  88
531  94
532  96
533  94
534  86
535  97
536  84
537  95
538  94
539  99
540  99
541  95
542  99
543  93
544  97
545  95
546  98
547  90
548  99
549  91
550  95
551  99
552  99
553  94
554  98
555  94
556  97
557  98
558  77
559  97
560  98
561  92
562  98
563  90
564  99
565  92
566  92
567  88
568  97
569  94
570  98
571  97
572  93
573  98
574  99
575  93
576  98
577  99
578  98
579  95
580  87
581  98
582  93
583  92
584  86
585  85
586  99
587  99
588  99
589  98
590  95
591  91
592  98
593  98
594  96
595  96
596  99
597  87
598  97
599  93
600  94
601  97
602  94
603  99
604  99
605  98
606  98
607  99
608  99
609  97
610  99
611  99
612  93
613  97
614  90
615  90
616  99
617  96
618  98
619  99
620  96
621  96
622  92
623  94
624  89
625  95
626  93
627  93
628  94
629  94
630  99
631  96
632  97
633  96
634  60
635  87
636  99
637  98
638  97
639  94
640  97
641  98
642  94
643  95
644  77
645  95
646  89
647  96
648  91
649  97
650  91
651  88
652  92
653  97
654  99
655  94
656  95
657  97
658  99
659  78
660  98
661  93
662  92
663  95
664  97
665  94
666  95
667  98
668  94
669  93
670  97
671  96
672  84
673  98
674  95
675  90
676  96
677  85
678  95
679  99
680  89
681  86
682  92
683  89
684  96
685  97
686  97
687  95
688  97
689  94
690  98
691  86
692  84
693  98
694  98
695  88
696  97
697  93
698  88
699  98
700  96
701  97
702  96
703  97
704  97
705  97
706  84
707  97
708  97
709  93
710  98
711  98
712  94
713  98
714  94
715  82
716  99
717  96
718  98
719  97
720  99
721  97
722  98
723  98
724  87
725  96
726  99
727  90
728  96
729  99
730  96
731  99
732  96
733  97
734  99
735  98
736  98
737  97
738  97
739  98
740  94
741  98
742  96
743  98
744  92
745  96
746  97
747  98
748  94
749  88
750  96
751  98
752  99
753  98
754  99
755  97
756  92
757  96
758  87
759  99
760  98
761  96
762  95
763  94
764  98
765  94
766  97
767  97
768  99
769  98
770  77
771  89
772  90
773  99
774  99
775  96
776  84
777  95
778  96
779  97
780  97
781  99
782  99
783  93
784  98
785  95
786  97
787  97
788  99
789  99
790  94
791  83
792  91
793  94
794  99
795  98
796  88
797  98
798  95
799  90
800  98
801  98
802  94
803  99
804  92
805  99
806  91
807  93
808  94
809  94
810  85
811  95
812  89
813  97
814  96
815  94
816  90
817  95
818  85
819  94
820  83
821  96
822  97
823  98
824  99
825  97
826  96
827  94
828  93
829  95
830  90
831  99
832  82
833  98
834  89
835  96
836  95
837  93
838  99
839  88
840  97
841  98
842  97
843  99
844  96
845  97
846  96
847  99
848  92
849  92
850  97
851  99
852  94
853  94
854  92
855  89
856  98
857  98
858  96
859  99
860  93
861  95
862  99
863  97
864  98
865  99
866  95
867  89
868  82
869  98
870  99
871  97
872  93
873  96
874  99
875  99
876  85
877  91
878  90
879  99
880  99
881  96
882  98
883  97
884  95
885  97
886  95
887  94
888  97
889  96
890  91
891  98
892  94
893  96
894  91
895  99
896  97
897  92
898  94
899  90
900  96
901  96
902  99
903  93
904  97
905  91
906  81
907  98
908  75
909  95
910  97
911  85
912  93
913  98
914  97
915  93
916  86
917  95
918  99
919  98
920  78
921  74
922  98
923  99
924  98
925  97
926  98
927  99
928  99
929  98
930  99
931  96
932  94
933  87
934  97
935  88
936  94
937  82
938  92
939  79
940  94
941  97
942  81
943  97
944  99
945  98
946  98
947  99
948  99
949  99
950  98
951  99
952  98
953  94
954  98
955  94
956  82
957  95
958  98
959  94
960  97
961  93
962  99
963  99
964  95
965  91
966  96
967  99
968  97
969  79
970  91
971  97
972  90
973  94
974  98
975  97
976  87
977  92
978  88
979  83
980  99
981  98
982  95
983  89
984  98
985  94
986  96
987  82
988  94
989  97
990  98
991  98
992  97
993  99
994  98
995  96
996  94
997  98
998  94
999  94
1000  99
1001  96
1002  97
1003  96
1004  94
1005  98
1006  88
1007  93
1008  98
1009  96
1010  88
1011  91
1012  79
1013  84
1014  89
1015  92
1016  98
1017  98
1018  99
1019  98
1020  98
1021  85
1022  98
1023  85
1024  95
1025  91
1026  96
1027  95
1028  99
1029  99
1030  99
1031  87
1032  90
1033  99
1034  95
1035  78
1036  90
1037  98
1038  97
1039  96
1040  98
1041  88
1042  95
1043  96
1044  98
1045  96
1046  93
1047  98
1048  98
1049  95
1050  96
1051  93
1052  95
1053  99
1054  97
1055  97
1056  85
1057  81
1058  77
1059  97
1060  97
1061  94
1062  98
1063  94
1064  99
1065  97
1066  98
1067  94
1068  96
1069  97
1070  99
1071  96
1072  99
1073  99
1074  99
1075  95
1076  95
1077  95
1078  99
1079  92
1080  91
1081  98
1082  92
1083  98
1084  98
1085  98
1086  97
1087  99
1088  99
1089  95
1090  94
1091  99
1092  96
1093  89
1094  96
1095  92
1096  94
1097  95
1098  97
1099  97
1100  96
1101  97
1102  96
1103  93
1104  98
1105  99
1106  85
1107  93
1108  97
1109  98
1110  98
1111  94
1112  84
1113  99
1114  99
1115  87
1116  98
1117  88
1118  98
1119  97
1120  96
1121  97
1122  99
1123  96
1124  99
1125  83
1126  98
1127  98
1128  90
1129  99
1130  97
1131  99
1132  97
1133  98
1134  98
1135  93
1136  99
1137  97
1138  92
1139  98
1140  90
1141  95
1142  85
1143  85
1144  98
1145  91
1146  95
1147  90
1148  97
1149  88
1150  94
1151  85
1152  88
1153  97
1154  95
1155  99
1156  91
1157  99
1158  99
1159  94
1160  94
1161  96
1162  90
1163  98
1164  94
1165  93
1166  94
1167  96
1168  96
1169  99
1170  98
1171  95
1172  85
1173  96
1174  95
1175  91
1176  97
1177  96
1178  99
1179  97
1180  95
1181  98
1182  98
1183  99
1184  76
1185  91
1186  89
1187  98
1188  99
1189  92
1190  87
1191  98
1192  96
1193  97
1194  84
1195  96
1196  99
1197  91
1198  95
1199  99
1200  93
1201  98
1202  98
1203  98
1204  86
1205  97
1206  97
1207  94
1208  97
1209  99
1210  94
1211  89
1212  81
1213  99
1214  75
1215  99
1216  96
1217  92
1218  97
1219  98
1220  96
1221  94
1222  99
1223  92
1224  99
1225  98
1226  88
1227  96
1228  96
1229  98
1230  98
1231  99
1232  99
1233  92
1234  95
1235  96
1236  97
1237  88
1238  99
1239  93
1240  99
1241  90
1242  93
1243  99
1244  90
1245  99
1246  89
1247  93
1248  89
1249  99
1250  99
1251  75
1252  80
1253  99
1254  97
1255  97
1256  98
1257  98
1258  94
1259  92
1260  97
1261  97
1262  99
1263  98
1264  98
1265  94
1266  97
1267  90
1268  96
1269  93
1270  94
1271  97
1272  98
1273  94
1274  98
1275  74
1276  80
1277  96
1278  97
1279  98
1280  93
1281  99
1282  93
1283  99
1284  98
1285  95
1286  95
1287  91
1288  94
1289  88
1290  98
1291  93
1292  96
1293  86
1294  97
1295  95
1296  96
1297  96
1298  85
1299  79
1300  92
1301  92
1302  98
1303  98
1304  93
1305  97
1306  88
1307  94
1308  82
1309  99
1310  98
1311  99
1312  95
1313  95
1314  99
1315  99
1316  92
1317  99
1318  91
1319  98
1320  98
1321  90
1322  99
1323  99
1324  96
1325  91
1326  99
1327  99
1328  90
1329  90
1330  96
1331  97
1332  96
1333  98
1334  96
1335  96
1336  96
1337  98
1338  95
1339  90
1340  94
1341  98
1342  94
1343  95
1344  74
1345  96
1346  87
1347  97
1348  95
1349  99
1350  96
1351  75
1352  98
1353  94
1354  98
1355  94
1356  92
1357  96
1358  95
1359  98
1360  94
1361  98
1362  99
1363  89
1364  97
1365  93
1366  88
1367  91
1368  95
1369  87
1370  99
1371  97
1372  94
1373  97
1374  96
1375  98
1376  99
1377  98
1378  99
1379  88
1380  99
1381  99
1382  94
1383  88
1384  94
1385  92
1386  96
1387  99
1388  99
1389  99
1390  99
1391  98
1392  97
1393  98
1394  97
1395  98
1396  94
1397  99
1398  95
1399  75
1400  93
1401  97
1402  97
1403  95
1404  94
1405  97
1406  92
1407  99
1408  97
1409  97
1410  68
1411  66
1412  83
1413  96
1414  85
1415  96
1416  98
1417  99
1418  99
1419  99
1420  98
1421  89
1422  99
1423  85
1424  96
1425  83
1426  99
1427  84
1428  72
1429  90
1430  90
1431  98
1432  98
1433  98
1434  95
1435  94
1436  99
1437  85
1438  73
1439  93
1440  98
1441  97
1442  96
1443  92
1444  99
1445  98
1446  97
1447  99
1448  99
1449  98
1450  99
1451  91
1452  98
1453  97
1454  90
1455  98
1456  99
1457  95
1458  97
1459  99
1460  97
1461  92
1462  97
1463  97
1464  98
1465  99
1466  88
1467  95
1468  99
1469  98
1470  84
1471  92
1472  97
1473  99
1474  87
1475  97
1476  98
1477  95
1478  82
1479  81
1480  97
1481  97
1482  94
1483  96
1484  99
1485  99
1486  99
1487  99
1488  99
1489  98
1490  95
1491  94
1492  98
1493  83
1494  98
1495  96
1496  97
1497  92
1498  87
1499  86
1500  93
1501  81
1502  88
1503  96
1504  99
1505  86
1506  93
1507  94
1508  84
1509  90
1510  98
1511  94
1512  97
1513  97
1514  92
1515  97
1516  95
1517  99
1518  99
1519  98
1520  91
1521  89
1522  85
1523  84
1524  96
1525  92
1526  98
1527  96
1528  92
1529  97
1530  91
1531  98
1532  98
1533  86
1534  98
1535  97
1536  99
1537  89
1538  99
1539  97
1540  98
1541  96
1542  95
1543  94
1544  96
1545  93
1546  91
1547  95
1548  99
1549  95
1550  99
1551  85
1552  90
1553  99
1554  88
1555  99
1556  98
1557  97
1558  98
1559  95
1560  96
1561  88
1562  86
1563  95
1564  94
1565  99
1566  96
1567  99
1568  97
1569  98
1570  80
1571  95
1572  97
1573  98
1574  99
1575  98
1576  98
1577  97
1578  93
1579  98
1580  99
1581  97
1582  91
1583  98
1584  80
1585  81
1586  96
1587  98
1588  90
1589  95
1590  97
1591  94
1592  98
1593  97
1594  98
1595  96
1596  91
1597  98
1598  97
1599  96
1600  96
1601  98
1602  98
1603  97
1604  92
1605  99
1606  94
1607  97
1608  95
1609  99
1610  99
1611  98
1612  99
1613  92
1614  87
1615  97
1616  99
1617  88
1618  99
1619  97
1620  92
1621  99
1622  96
1623  99
1624  91
1625  87
1626  99
1627  96
1628  98
1629  98
1630  92
1631  96
1632  95
1633  98
1634  99
1635  98
1636  92
1637  95
1638  96
1639  97
1640  96
1641  96
1642  99
1643  99
1644  93
1645  96
1646  93
1647  97
1648  95
1649  93
1650  97
1651  99
1652  98
1653  95
1654  98
1655  96
1656  90
1657  93
1658  99
1659  97
1660  95
1661  87
1662  99
1663  99
1664  97
1665  94
1666  90
1667  95
1668  95
1669  91
1670  97
1671  87
1672  75
1673  99
1674  93
1675  82
1676  99
1677  97
1678  97
1679  91
1680  97
1681  98
1682  98
1683  98
1684  92
1685  95
1686  99
1687  95
1688  98
1689  97
1690  95
1691  95
1692  98
1693  98
1694  91
1695  81
1696  85
1697  93
1698  97
1699  84
1700  97
1701  93
1702  90
1703  97
1704  90
1705  99
1706  96
1707  97
1708  98
1709  92
1710  91
1711  98
1712  99
1713  94
1714  96
1715  98
1716  94
1717  98
1718  95
1719  88
1720  98
1721  99
1722  98
1723  99
1724  93
1725  96
1726  92
1727  93
1728  99
1729  97
1730  95
1731  92
1732  95
1733  89
1734  94
1735  88
1736  98
1737  97
1738  97
1739  96
1740  90
1741  96
1742  99
1743  97
1744  92
1745  97
1746  98
1747  96
1748  99
1749  96
1750  99
1751  98
1752  99
1753  99
1754  99
1755  99
1756  96
1757  98
1758  96
1759  99
1760  99
1761  96
1762  99
1763  99
1764  98
1765  86
1766  97
1767  89
1768  86
1769  80
1770  93
1771  98
1772  97
1773  98
1774  96
1775  93
1776  94
1777  99
1778  99
1779  90
1780  99
1781  99
1782  98
1783  93
1784  92
1785  99
1786  98
1787  95
1788  97
1789  98
1790  98
1791  94
1792  86
1793  93
1794  83
1795  97
1796  97
1797  98
1798  85
1799  98
1800  94
1801  79
1802  98
1803  96
1804  98
1805  98
1806  98
1807  97
1808  95
1809  99
1810  95
1811  97
1812  97
1813  94
1814  98
1815  95
1816  98
1817  96
1818  97
1819  95
1820  94
1821  98
1822  98
1823  93
1824  92
1825  92
1826  93
1827  88
1828  97
1829  97
1830  96
1831  97
1832  93
1833  96
1834  97
1835  99
1836  97
1837  97
1838  99
1839  97
1840  99
1841  94
1842  96
1843  97
1844  96
1845  98
1846  97
1847  99
1848  99
1849  96
1850  73
1851  66
1852  97
1853  96
1854  94
1855  99
1856  99
1857  96
1858  94
1859  97
1860  88
1861  99
1862  94
1863  95
1864  97
1865  95
1866  97
1867  99
1868  99
1869  95
1870  82
1871  94
1872  95
1873  90
1874  99
1875  97
1876  95
1877  85
1878  99
1879  99
1880  92
1881  90
1882  98
1883  81
1884  97
1885  97
1886  96
1887  97
1888  99
1889  95
1890  91
1891  98
1892  92
1893  87
1894  97
1895  93
1896  95
1897  98
1898  98
1899  98
1900  94
1901  85
1902  91
1903  98
1904  97
1905  93
1906  98
1907  94
1908  90
1909  99
1910  89
1911  95
1912  99
1913  97
1914  97
1915  99
1916  86
1917  98
1918  96
1919  99
1920  99
1921  95
1922  99
1923  98
1924  99
1925  94
1926  97
1927  86
1928  99
1929  96
1930  98
1931  91
1932  98
1933  95
1934  96
1935  94
1936  99
1937  91
1938  97
1939  91
1940  98
1941  96
1942  91
1943  97
1944  98
1945  97
1946  98
1947  96
1948  99
1949  95
1950  93
1951  98
1952  96
1953  95
1954  96
1955  90
1956  96
1957  94
1958  98
1959  98
1960  99
1961  96
1962  99
1963  78
1964  96
1965  96
1966  98
1967  92
1968  94
1969  95
1970  95
1971  99
1972  75
1973  88
1974  82
1975  84
1976  85
1977  97
1978  89
1979  96
1980  97
1981  94
1982  98
1983  98
1984  94
1985  77
1986  99
1987  98
1988  99
1989  99
1990  96
1991  95
1992  98
1993  95
1994  94
1995  90
1996  97
1997  99
1998  97
1999  82
2000  99
2001  94

==> data/used_slots_dscf_100_multithr_2_25_9_8.tex <==
idx  slots
1  10
2  12
3  27
4  6
5  5
6  12
7  15
8  12
9  15
10  29
11  53
12  56
13  49
14  53
15  42
16  33
17  24
18  23
19  20
20  8
21  11
22  12
23  9
24  9
25  20
26  41
27  40
28  29
29  42
30  27
31  25
32  20
33  24
34  21
35  4
36  11
37  15
38  19
39  12
40  10
41  15
42  26
43  41
44  49
45  40
46  43
47  44
48  49
49  43
50  42
51  49
52  42
53  49
54  42
55  43
56  57
57  54
58  50
59  56
60  39
61  45
62  34
63  39
64  42
65  35
66  44
67  59
68  44
69  47
70  66
71  64
72  55
73  48
74  48
75  49
76  47
77  49
78  62
79  47
80  30
81  45
82  32
83  44
84  53
85  48
86  44
87  48
88  51
89  53
90  47
91  60
92  63
93  58
94  56
95  60
96  48
97  53
98  46
99  42
100  28
101  34
102  23
103  4
104  32
105  32
106  27
107  23
108  27
109  29
110  23
111  22
112  21
113  22
114  18
115  23
116  16
117  31
118  34
119  22
120  22
121  32
122  34
123  36
124  46
125  27
126  38
127  39
128  29
129  20
130  16
131  18
132  7
133  9
134  8
135  11
136  7
137  9
138  14
139  15
140  4
141  11
142  5
143  31
144  48
145  45
146  52
147  52
148  38
149  49
150  47
151  48
152  50
153  42
154  41
155  29
156  11
157  20
158  21
159  21
160  11
161  23
162  25
163  30
164  44
165  33
166  21
167  29
168  27
169  37
170  35
171  34
172  54
173  51
174  55
175  52
176  57
177  69
178  71
179  70
180  62
181  52
182  34
183  37
184  38
185  43
186  34
187  36
188  24
189  20
190  24
191  16
192  11
193  21
194  22
195  14
196  21
197  19
198  13
199  23
200  30
201  24
202  36
203  35
204  25
205  14
206  13
207  6
208  12
209  27
210  27
211  17
212  13
213  18
214  35
215  30
216  38
217  53
218  42
219  39
220  30
221  46
222  63
223  46
224  51
225  46
226  43
227  46
228  50
229  51
230  62
231  43
232  43
233  49
234  52
235  39
236  41
237  47
238  45
239  50
240  37
241  43
242  53
243  42
244  35
245  40
246  46
247  30
248  34
249  40
250  42
251  40
252  33
253  18
254  34
255  48
256  34
257  16
258  29
259  29
260  28
261  27
262  37
263  31
264  34
265  38
266  37
267  49
268  52
269  48
270  47
271  55
272  50
273  45
274  46
275  31
276  31
277  38
278  39
279  24
280  22
281  35
282  50
283  50
284  44
285  38
286  48
287  49
288  46
289  40
290  46
291  36
292  35
293  18
294  17
295  9
296  17
297  23
298  33
299  39
300  47
301  46
302  35
303  35
304  28
305  16
306  14
307  9
308  11
309  27
310  41
311  37
312  56
313  56
314  41
315  50
316  61
317  47
318  55
319  54
320  49
321  49
322  39
323  52
324  49
325  47
326  33
327  28
328  23
329  20
330  24
331  21
332  28
333  42
334  44
335  58
336  45
337  46
338  33
339  38
340  51
341  38
342  53
343  47
344  38
345  35
346  31
347  50
348  44
349  48
350  49
351  39
352  35
353  39
354  48
355  28
356  29
357  22
358  40
359  28
360  43
361  36
362  29
363  29
364  40
365  34
366  35
367  33
368  39
369  40
370  16
371  16
372  32
373  32
374  38
375  32
376  33
377  45
378  19
379  29
380  31
381  21
382  14
383  20
384  9
385  32
386  26
387  42
388  36
389  30
390  19
391  10
392  20
393  7
394  8
395  14
396  28
397  45
398  49
399  53
400  46
401  32
402  35
403  12
404  4
405  6
406  20
407  13
408  15
409  11
410  6
411  7
412  8
413  15
414  20
415  26
416  44
417  44
418  36
419  34
420  46
421  47
422  55
423  54
424  63
425  57
426  55
427  51
428  50
429  62
430  58
431  43
432  41
433  49
434  46
435  42
436  40
437  43
438  44
439  42
440  34
441  54
442  58
443  46
444  40
445  46
446  36
447  39
448  35
449  44
450  47
451  49
452  60
453  56
454  46
455  38
456  47
457  43
458  44
459  28
460  31
461  28
462  38
463  47
464  47
465  50
466  54
467  49
468  55
469  40
470  53
471  51
472  50
473  40
474  64
475  65
476  64
477  64
478  52
479  41
480  45
481  52
482  45
483  47
484  51
485  38
486  43
487  41
488  41
489  49
490  35
491  20
492  17
493  12
494  11
495  17
496  21
497  29
498  44
499  45
500  50
501  54
502  47
503  50
504  44
505  28
506  43
507  43
508  38
509  52
510  37
511  19
512  35
513  42
514  48
515  54
516  49
517  42
518  56
519  46
520  37
521  28
522  33
523  40
524  35
525  39
526  52
527  45
528  71
529  62
530  56
531  52
532  46
533  34
534  25
535  29
536  18
537  26
538  16
539  26
540  48
541  48
542  49
543  41
544  28
545  46
546  52
547  46
548  61
549  61
550  70
551  70
552  78
553  81
554  81
555  77
556  59
557  57
558  37
559  44
560  46
561  42
562  54
563  53
564  56
565  61
566  54
567  40
568  36
569  23
570  31
571  28
572  22
573  25
574  34
575  42
576  52
577  57
578  62
579  61
580  42
581  53
582  47
583  40
584  25
585  15
586  20
587  28
588  24
589  19
590  20
591  19
592  28
593  45
594  47
595  38
596  54
597  41
598  46
599  56
600  48
601  63
602  69
603  70
604  86
605  76
606  72
607  66
608  66
609  75
610  67
611  63
612  54
613  52
614  50
615  32
616  47
617  50
618  45
619  51
620  44
621  51
622  64
623  60
624  43
625  44
626  38
627  46
628  49
629  45
630  65
631  59
632  53
633  45
634  9
635  13
636  16
637  15
638  10
639  9
640  19
641  33
642  33
643  46
644  26
645  29
646  22
647  21
648  20
649  27
650  20
651  11
652  21
653  15
654  29
655  27
656  16
657  15
658  26
659  8
660  12
661  15
662  15
663  27
664  37
665  28
666  34
667  43
668  51
669  47
670  63
671  56
672  42
673  45
674  50
675  39
676  37
677  32
678  32
679  56
680  47
681  37
682  37
683  33
684  41
685  49
686  49
687  38
688  33
689  39
690  50
691  32
692  33
693  53
694  48
695  30
696  27
697  9
698  16
699  18
700  24
701  20
702  16
703  13
704  12
705  15
706  9
707  19
708  18
709  15
710  12
711  14
712  24
713  22
714  8
715  13
716  17
717  28
718  14
719  18
720  30
721  18
722  39
723  48
724  38
725  29
726  37
727  36
728  45
729  50
730  51
731  44
732  55
733  59
734  65
735  53
736  46
737  48
738  45
739  43
740  35
741  38
742  26
743  28
744  21
745  29
746  37
747  49
748  44
749  36
750  37
751  37
752  35
753  33
754  55
755  47
756  38
757  44
758  26
759  39
760  36
761  33
762  33
763  34
764  39
765  42
766  43
767  48
768  52
769  44
770  27
771  29
772  23
773  13
774  17
775  5
776  14
777  13
778  17
779  26
780  18
781  27
782  51
783  42
784  31
785  18
786  11
787  10
788  13
789  35
790  23
791  6
792  12
793  25
794  31
795  33
796  21
797  49
798  53
799  39
800  42
801  58
802  52
803  53
804  45
805  42
806  30
807  26
808  25
809  18
810  15
811  27
812  30
813  50
814  46
815  48
816  42
817  42
818  30
819  25
820  15
821  13
822  15
823  22
824  25
825  19
826  22
827  31
828  34
829  28
830  22
831  31
832  6
833  30
834  20
835  22
836  19
837  28
838  28
839  12
840  15
841  10
842  17
843  24
844  22
845  12
846  24
847  26
848  21
849  12
850  16
851  32
852  31
853  27
854  19
855  9
856  13
857  12
858  18
859  38
860  36
861  35
862  27
863  37
864  37
865  38
866  41
867  26
868  18
869  26
870  18
871  12
872  15
873  14
874  27
875  35
876  34
877  21
878  13
879  17
880  21
881  18
882  28
883  23
884  30
885  22
886  32
887  43
888  47
889  36
890  28
891  45
892  30
893  30
894  20
895  17
896  18
897  16
898  15
899  16
900  28
901  32
902  44
903  56
904  60
905  54
906  36
907  36
908  10
909  22
910  29
911  16
912  9
913  9
914  24
915  29
916  33
917  21
918  38
919  48
920  33
921  24
922  44
923  49
924  49
925  37
926  32
927  37
928  37
929  52
930  56
931  54
932  49
933  51
934  54
935  45
936  50
937  37
938  26
939  4
940  13
941  21
942  12
943  28
944  25
945  23
946  25
947  23
948  28
949  43
950  41
951  45
952  47
953  46
954  52
955  54
956  38
957  47
958  51
959  47
960  45
961  51
962  52
963  53
964  56
965  46
966  41
967  47
968  40
969  21
970  9
971  23
972  25
973  35
974  30
975  35
976  35
977  34
978  13
979  13
980  30
981  38
982  39
983  19
984  23
985  32
986  36
987  18
988  12
989  8
990  26
991  31
992  30
993  41
994  39
995  45
996  43
997  45
998  44
999  43
1000  46
1001  31
1002  33
1003  45
1004  56
1005  45
1006  41
1007  30
1008  42
1009  50
1010  45
1011  35
1012  14
1013  11
1014  10
1015  12
1016  17
1017  20
1018  15
1019  22
1020  48
1021  38
1022  30
1023  22
1024  19
1025  21
1026  31
1027  21
1028  24
1029  39
1030  43
1031  43
1032  51
1033  54
1034  42
1035  26
1036  32
1037  61
1038  56
1039  46
1040  49
1041  35
1042  35
1043  22
1044  19
1045  35
1046  30
1047  24
1048  20
1049  37
1050  27
1051  18
1052  19
1053  33
1054  31
1055  47
1056  29
1057  20
1058  11
1059  20
1060  15
1061  33
1062  39
1063  31
1064  22
1065  13
1066  18
1067  11
1068  25
1069  19
1070  28
1071  23
1072  19
1073  37
1074  37
1075  31
1076  15
1077  16
1078  16
1079  19
1080  13
1081  16
1082  11
1083  26
1084  33
1085  35
1086  49
1087  57
1088  55
1089  64
1090  72
1091  78
1092  66
1093  52
1094  58
1095  34
1096  30
1097  11
1098  21
1099  33
1100  36
1101  49
1102  58
1103  52
1104  57
1105  55
1106  47
1107  46
1108  45
1109  49
1110  46
1111  46
1112  30
1113  36
1114  43
1115  30
1116  52
1117  40
1118  59
1119  54
1120  48
1121  48
1122  52
1123  49
1124  52
1125  35
1126  51
1127  52
1128  51
1129  36
1130  53
1131  50
1132  56
1133  52
1134  46
1135  47
1136  46
1137  42
1138  34
1139  52
1140  38
1141  44
1142  38
1143  27
1144  16
1145  20
1146  4
1147  9
1148  19
1149  13
1150  23
1151  14
1152  8
1153  28
1154  11
1155  17
1156  18
1157  10
1158  16
1159  25
1160  23
1161  9
1162  10
1163  10
1164  14
1165  22
1166  18
1167  29
1168  25
1169  31
1170  21
1171  20
1172  8
1173  20
1174  12
1175  6
1176  12
1177  19
1178  22
1179  22
1180  24
1181  41
1182  50
1183  48
1184  28
1185  18
1186  3
1187  8
1188  29
1189  11
1190  7
1191  22
1192  33
1193  33
1194  20
1195  24
1196  24
1197  35
1198  33
1199  28
1200  22
1201  44
1202  37
1203  36
1204  16
1205  17
1206  9
1207  24
1208  22
1209  27
1210  43
1211  34
1212  27
1213  32
1214  15
1215  27
1216  29
1217  29
1218  41
1219  52
1220  57
1221  53
1222  57
1223  61
1224  62
1225  67
1226  54
1227  55
1228  48
1229  40
1230  40
1231  39
1232  51
1233  39
1234  55
1235  43
1236  38
1237  40
1238  38
1239  40
1240  48
1241  49
1242  36
1243  33
1244  24
1245  23
1246  12
1247  11
1248  14
1249  34
1250  37
1251  22
1252  13
1253  17
1254  27
1255  19
1256  34
1257  46
1258  38
1259  25
1260  28
1261  34
1262  33
1263  30
1264  11
1265  16
1266  16
1267  10
1268  12
1269  8
1270  12
1271  20
1272  34
1273  15
1274  7
1275  7
1276  9
1277  14
1278  10
1279  15
1280  8
1281  17
1282  12
1283  25
1284  29
1285  30
1286  22
1287  13
1288  12
1289  11
1290  17
1291  6
1292  15
1293  8
1294  7
1295  12
1296  8
1297  11
1298  10
1299  13
1300  22
1301  17
1302  39
1303  32
1304  31
1305  31
1306  24
1307  28
1308  15
1309  29
1310  44
1311  51
1312  41
1313  42
1314  40
1315  42
1316  38
1317  46
1318  43
1319  45
1320  48
1321  51
1322  40
1323  42
1324  48
1325  50
1326  50
1327  52
1328  42
1329  31
1330  29
1331  32
1332  23
1333  23
1334  27
1335  18
1336  33
1337  33
1338  45
1339  30
1340  26
1341  30
1342  18
1343  35
1344  12
1345  14
1346  10
1347  20
1348  24
1349  24
1350  24
1351  4
1352  20
1353  15
1354  19
1355  9
1356  10
1357  12
1358  19
1359  30
1360  26
1361  41
1362  48
1363  44
1364  44
1365  37
1366  29
1367  33
1368  34
1369  20
1370  18
1371  16
1372  7
1373  28
1374  42
1375  58
1376  54
1377  51
1378  52
1379  45
1380  37
1381  49
1382  41
1383  33
1384  36
1385  35
1386  34
1387  34
1388  43
1389  48
1390  36
1391  41
1392  46
1393  50
1394  51
1395  42
1396  27
1397  35
1398  43
1399  17
1400  13
1401  21
1402  41
1403  27
1404  15
1405  22
1406  8
1407  11
1408  25
1409  39
1410  10
1411  7
1412  11
1413  6
1414  15
1415  13
1416  13
1417  28
1418  37
1419  45
1420  51
1421  50
1422  51
1423  42
1424  40
1425  15
1426  25
1427  4
1428  5
1429  15
1430  6
1431  11
1432  30
1433  39
1434  37
1435  38
1436  54
1437  41
1438  25
1439  23
1440  26
1441  27
1442  29
1443  25
1444  18
1445  25
1446  19
1447  22
1448  32
1449  48
1450  48
1451  50
1452  50
1453  49
1454  43
1455  50
1456  53
1457  58
1458  53
1459  58
1460  65
1461  51
1462  52
1463  44
1464  51
1465  53
1466  43
1467  50
1468  46
1469  53
1470  37
1471  36
1472  46
1473  37
1474  17
1475  12
1476  17
1477  8
1478  6
1479  9
1480  10
1481  16
1482  31
1483  33
1484  55
1485  62
1486  51
1487  50
1488  56
1489  57
1490  51
1491  48
1492  56
1493  34
1494  37
1495  41
1496  48
1497  49
1498  40
1499  30
1500  29
1501  9
1502  14
1503  23
1504  28
1505  14
1506  13
1507  38
1508  21
1509  26
1510  38
1511  32
1512  23
1513  17
1514  17
1515  24
1516  30
1517  31
1518  45
1519  39
1520  43
1521  41
1522  31
1523  20
1524  14
1525  19
1526  27
1527  24
1528  38
1529  37
1530  44
1531  43
1532  47
1533  36
1534  30
1535  28
1536  26
1537  22
1538  42
1539  48
1540  53
1541  50
1542  47
1543  39
1544  31
1545  28
1546  23
1547  15
1548  17
1549  20
1550  23
1551  15
1552  10
1553  9
1554  10
1555  34
1556  49
1557  50
1558  47
1559  56
1560  49
1561  28
1562  20
1563  26
1564  28
1565  32
1566  35
1567  29
1568  35
1569  33
1570  20
1571  19
1572  26
1573  35
1574  37
1575  37
1576  46
1577  50
1578  45
1579  49
1580  51
1581  51
1582  42
1583  49
1584  36
1585  21
1586  35
1587  22
1588  12
1589  20
1590  6
1591  15
1592  13
1593  12
1594  21
1595  45
1596  43
1597  52
1598  41
1599  39
1600  35
1601  28
1602  40
1603  40
1604  32
1605  42
1606  40
1607  50
1608  46
1609  41
1610  39
1611  60
1612  50
1613  40
1614  25
1615  23
1616  27
1617  12
1618  35
1619  37
1620  39
1621  54
1622  49
1623  77
1624  61
1625  50
1626  57
1627  58
1628  60
1629  50
1630  41
1631  39
1632  38
1633  32
1634  43
1635  39
1636  29
1637  33
1638  48
1639  54
1640  54
1641  64
1642  63
1643  58
1644  72
1645  61
1646  50
1647  61
1648  59
1649  42
1650  61
1651  68
1652  63
1653  54
1654  58
1655  65
1656  55
1657  44
1658  46
1659  49
1660  48
1661  35
1662  35
1663  45
1664  42
1665  56
1666  55
1667  49
1668  52
1669  31
1670  36
1671  18
1672  9
1673  9
1674  14
1675  9
1676  24
1677  20
1678  25
1679  16
1680  34
1681  37
1682  32
1683  38
1684  33
1685  43
1686  50
1687  47
1688  64
1689  61
1690  52
1691  43
1692  48
1693  53
1694  42
1695  28
1696  27
1697  31
1698  34
1699  21
1700  33
1701  29
1702  18
1703  30
1704  13
1705  30
1706  43
1707  40
1708  36
1709  33
1710  36
1711  42
1712  50
1713  45
1714  43
1715  45
1716  50
1717  50
1718  43
1719  44
1720  40
1721  52
1722  53
1723  48
1724  49
1725  42
1726  47
1727  46
1728  45
1729  33
1730  44
1731  48
1732  43
1733  40
1734  35
1735  26
1736  21
1737  11
1738  16
1739  15
1740  13
1741  13
1742  23
1743  30
1744  20
1745  36
1746  39
1747  49
1748  47
1749  44
1750  42
1751  48
1752  52
1753  54
1754  53
1755  48
1756  46
1757  57
1758  50
1759  57
1760  57
1761  51
1762  52
1763  68
1764  65
1765  53
1766  47
1767  38
1768  26
1769  16
1770  20
1771  13
1772  11
1773  13
1774  9
1775  6
1776  4
1777  7
1778  14
1779  16
1780  28
1781  32
1782  44
1783  52
1784  42
1785  44
1786  44
1787  53
1788  46
1789  48
1790  56
1791  61
1792  47
1793  37
1794  29
1795  32
1796  39
1797  35
1798  31
1799  58
1800  53
1801  26
1802  29
1803  23
1804  22
1805  40
1806  48
1807  54
1808  54
1809  42
1810  41
1811  50
1812  52
1813  47
1814  57
1815  58
1816  61
1817  60
1818  49
1819  37
1820  33
1821  39
1822  36
1823  37
1824  44
1825  54
1826  47
1827  37
1828  38
1829  50
1830  47
1831  39
1832  33
1833  25
1834  47
1835  50
1836  64
1837  72
1838  65
1839  65
1840  66
1841  69
1842  63
1843  62
1844  51
1845  52
1846  52
1847  60
1848  52
1849  50
1850  25
1851  14
1852  34
1853  25
1854  20
1855  48
1856  44
1857  45
1858  56
1859  46
1860  40
1861  57
1862  41
1863  45
1864  42
1865  39
1866  52
1867  64
1868  65
1869  58
1870  37
1871  34
1872  30
1873  16
1874  24
1875  28
1876  21
1877  10
1878  26
1879  28
1880  30
1881  16
1882  23
1883  7
1884  15
1885  20
1886  19
1887  19
1888  32
1889  23
1890  11
1891  10
1892  7
1893  9
1894  13
1895  3
1896  6
1897  10
1898  12
1899  17
1900  34
1901  15
1902  4
1903  11
1904  12
1905  18
1906  47
1907  58
1908  57
1909  59
1910  45
1911  33
1912  56
1913  44
1914  48
1915  42
1916  26
1917  34
1918  30
1919  38
1920  54
1921  57
1922  55
1923  71
1924  82
1925  67
1926  78
1927  69
1928  84
1929  88
1930  90
1931  82
1932  78
1933  68
1934  65
1935  54
1936  57
1937  57
1938  46
1939  33
1940  38
1941  45
1942  47
1943  45
1944  42
1945  43
1946  41
1947  37
1948  56
1949  51
1950  57
1951  54
1952  55
1953  53
1954  77
1955  63
1956  62
1957  49
1958  54
1959  52
1960  62
1961  53
1962  64
1963  45
1964  50
1965  44
1966  55
1967  49
1968  52
1969  49
1970  59
1971  55
1972  35
1973  27
1974  9
1975  6
1976  19
1977  18
1978  10
1979  18
1980  27
1981  33
1982  56
1983  46
1984  44
1985  25
1986  40
1987  48
1988  53
1989  53
1990  43
1991  43
1992  54
1993  40
1994  27
1995  12
1996  14
1997  11
1998  13
1999  8
2000  20
2001  26

==> diagrams/Buf_repres.tex <==
\begin{tikzpicture}
\node [draw, circle, align=center, inner sep=2mm, minimum width=3.5cm] (buf1) at (0.0,0) {};
\node [draw, circle, align=center, inner sep=2mm, minimum width=2.5cm] (buf2) at (0.0,0) {};

\draw [] (1.25,0.0) -- (1.75,0.0);
\draw [] (-1.25,0.0) -- (-1.75,0.0);
\draw [] (0.0, 1.25) -- (0.0, 1.75);
\draw [] (0.0, -1.25) -- (0.0, -1.75);
\draw [] (-0.8839, 0.8839) -- (-1.2374, 1.2374);
\draw [] (0.8839, 0.8839) -- (1.2374, 1.2374);
\draw [] (0.8839, -0.8839) -- (1.2374, -1.2374);
\draw [] (-0.8839, -0.8839) -- (-1.2374, -1.2374);

\node[] (lab0) at (0.5, 1.44){$0$};
\node[] (lab1) at (1.35, 0.6){$1$};
\node[] (lab2) at (1.4, -0.5){$2$};
\node[] (lab3) at (0.6, -1.4){$3$};
\node[] (lab4) at (-0.6, -1.35){$4$};
\node[] (lab5) at (-1.4, -0.5){$5$};
\node[] (lab6) at (-1.4, 0.55){$6$};
\node[] (lab7) at (-0.55, 1.44){$7$};

\draw [-latex] (0.0, 0.0) -- node[anchor=north]{\small{head}} (-0.9, 0.4);
\draw [-latex] (0.0, 0.0) -- node[anchor=south west]{\small{tail}} (0.4, -0.8);

\end{tikzpicture}

==> diagrams/Buf_time_diagram.tex <==
\begin{tikzpicture}[]
% time line
\draw (-3.2, 0.0) -- (4.4, 0.0);
% time steps
\draw (-3.0, -0.1) -- (-3.0, 0.1);
\draw (-2.6, -0.1) -- (-2.6, 0.1);
\draw (-2.2, -0.1) -- (-2.2, 0.1);
\draw (-1.8, -0.1) -- (-1.8, 0.1);
\draw (-1.4, -0.1) -- (-1.4, 0.1);
\draw (-1.0, -0.1) -- (-1.0, 0.1);
\draw (-0.6, -0.1) -- (-0.6, 0.1);
\draw (-0.2, -0.1) -- (-0.2, 0.1);
\draw (0.2, -0.1) -- (0.2, 0.1);
\draw (0.6, -0.1) -- (0.6, 0.1);
\draw (1.0, -0.1) -- (1.0, 0.1);
\draw (1.4, -0.1) -- (1.4, 0.1);
\draw (1.8, -0.1) -- (1.8, 0.1);
\draw (2.2, -0.1) -- (2.2, 0.1);
\draw (2.6, -0.1) -- (2.6, 0.1);
\draw (3.0, -0.1) -- (3.0, 0.1);
\draw (3.4, -0.1) -- (3.4, 0.1);
\draw (3.8, -0.1) -- (3.8, 0.1);
\draw (4.2, -0.1) -- (4.2, 0.1);

\node [] (story1) at (-3.6, 0.0){\ldots};
\node [] (story2) at (4.8, 0.0){\ldots};

\node [] (story3) at (-3.5, -1.6){\ldots};

\node [inner sep=1pt] (wr0) at (-3.0, 0.6){$w$};
\draw [-latex] (wr0) -- (-3.0, 0.0);

\node [inner sep=1pt] (wr1) at (-0.2, 0.6){$w$};
 \draw [-latex] (wr1) -- (-0.2, 0.0);
 \node [inner sep=1pt] (wr2) at (2.6, 0.6){$w$};
 \draw [-latex] (wr2) -- (2.6, 0.0);
 
 % reading definitions
\node [inner sep=1pt] (rd0) at (1.0, -0.6){$r$};
\draw [-latex] (1.0, 0.0) -- (rd0);
\node [inner sep=1pt] (rd1) at (3.0, -0.6){$r$};
\draw [-latex] (3.0, 0.0) -- (rd1);
 
\draw [dashed] (1.0, -0.8) -- (1.0, -1.6);
\draw [-latex] (-3.2, -1.6) -- node[anchor=south]{$t=11$, $\tau_{dec}=55$}(1.0, -1.6);
\draw [dashed] (3.0, -0.8) -- (3.0, -1.6);
\draw [-latex] (1.0, -1.6) -- node[anchor=south, align=center]{\small{$t\gets min\left(t_{cw},\,T_{max}\right)$} \\  \small{$\tau_{dec}=5$}}(3.0, -1.6);
 
 % controller detection
 \node [draw, ellipse, inner sep=0pt, minimum width=0.6cm, minimum height=0.5cm] (contrlab) at (-1.4, 1.2) {\small{$L_{free}<L_{thr,\,free}$}};
 \draw [-latex] (contrlab) -- (-1.4, 0.0);


\end{tikzpicture}

==> diagrams/SC_tree.tex <==
\begin{tikzpicture}[]

\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, label=south:{$\hat{u}_0$}] (u0) at (0,0){};
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, label=south:{$\hat{u}_1$}] (u1) at (0.6,0){};
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, label=south:{$\hat{u}_2$}] (u2) at (1.2,0){};
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, label=south:{$\hat{u}_3$}, fill=black] (u3) at (1.8,0){};
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, label=south:{$\hat{u}_4$}] (u4) at (2.4,0){};
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, label=south:{$\hat{u}_5$}, fill=black] (u5) at (3.0,0){};
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, label=south:{$\hat{u}_6$}, fill=black] (u6) at (3.6,0){};
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, label=south:{$\hat{u}_7$}, fill=black] (u7) at (4.2,0){};

\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, fill=gray!50!white] (n10) at (0.3,0.5){};
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, fill=gray!50!white] (n11) at (1.5,0.5){};
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, fill=gray!50!white] (n12) at (2.7,0.5){};
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, fill=gray!50!white] (n13) at (3.9,0.5){};
%
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, fill=gray!50!white] (n20) at (0.9,1.0){};
\node [draw, circle, color=green,  line width=0.8pt, inner sep=0.05 cm, fill=gray!50!white] (n21) at (3.3,1.0){\textcolor{black}{\footnotesize{$v$}}};
%
\node [draw, circle, line width=0.8pt, inner sep=0.1 cm, fill=gray!50!white] (n30) at (2.1,1.5){};
%
\draw (u0) -- node{}(n10);
\draw (u1) -- node{}(n10);
\draw (u2) -- node{}(n11);
\draw (u3) -- node{}(n11);
\draw (u4) -- node{}(n12);
\draw (u5) -- node{}(n12);
\draw (u6) -- node{}(n13);
\draw (u7) -- node{}(n13);
%
\draw [line width=0.8pt] (n10) -- node{}(n20);
\draw [line width=0.8pt] (n11) -- node{}(n20);
\draw [line width=0.8pt] (n12) -- node{}(n21);
\draw [line width=0.8pt] (n13) -- node{}(n21);
%
\draw [line width=1.2pt] (n20) -- node{}(n30);
\draw [line width=1.2pt] (n21) -- node{}(n30);
%
\draw [-latex] (2.3,1.56) -- node[anchor=south] {\footnotesize{$\alpha_v$}}(3.2,1.2);

\draw [-latex] (3.1,0.95) -- node{} (2.75,0.68);
\draw [-latex] (2.9,0.55) -- node{} (3.2,0.79);
\draw [-latex] (3.85,0.68) -- node{} (3.5,0.95);
\draw [-latex] (3.4,0.79) -- node{} (3.7,0.55);

\node [] (al) at (2.8,0.93){\footnotesize{$\alpha_l$}};
\node [] (ar) at (3.6,0.45){\footnotesize{$\alpha_r$}};
\node [] (bl) at (3.1,0.45){\footnotesize{$\beta_l$}};
\node [] (br) at (3.8,0.93){\footnotesize{$\beta_r$}};

\end{tikzpicture}


==> figures/Aver_Exec_Time/T_av_SCF_2_25.tex <==
\definecolor{MyDarkGreen}{HTML}{006100}
\definecolor{MyBlue}{rgb}{0.00000,0.44700,0.74100}%
\begin{tikzpicture}
  \pgfplotsset{
    label style = {font=\fontsize{9pt}{7.2}\selectfont},
    tick label style = {font=\fontsize{7pt}{7.2}\selectfont}
  }
   \begin{axis}[%
    width=\columnwidth,
    height=\plotfigureheight\columnwidth,
    bar shift auto,
    xmin=0, xmax=17,
    xtick={1,2,...,16},
    xlabel={Maximum number of trials $T_{init}$},
    xlabel style={yshift=0.4em},
    ymin=0.8, ymax=1.5,
    %ytick={0,1,2,...,10},
    ylabel style={yshift=-0.1em},
    ylabel={Average execution time $T_{av}$},
    xlabel style={yshift=-0.2em},
    %ylabel style={yshift=-1.0em},
    % yminorticks, xmajorgrids,
    ymajorgrids, %yminorgrids,
    legend style={legend columns=1},
    legend pos=south east,
    mark size=1.0pt, mark options=solid,
    ]    
    
    \addplot[ybar, bar width=0.5, fill=MyBlue,  draw=black] table[row sep=crcr]{%
      1 1.0\\
      2	1.066264\\
      3	1.117\\
      4	1.158926\\
      5	1.194821\\
      6	1.226346\\
      7	1.254433\\
      8	1.279851\\
      9 1.303094\\
      10 1.324559\\
      11 1.344505\\
      12 1.363073\\
      13 1.380573\\
      14 1.397104\\
      15 1.412735\\
      16 1.427637\\
      };
  
    \addplot[thick, samples=20,line width=1.0pt,  smooth,domain=0:16,red] coordinates {(1,1.3)(16,1.3)};
    
     \addplot[thick, samples=20,line width=1.0pt,  smooth,domain=0:16,MyDarkGreen] coordinates {(1,1.4)(16,1.4)};
    
    \node [](coef1) at (4.0,1.25)
    {\color{red}{\footnotesize{$\upsilon_{pr}=1.3$}}};
    
    \node [](coef2) at (4.0,1.42)
    {\color{MyDarkGreen}{\footnotesize{$\upsilon_{pr}=1.4$}}};
  
  \end{axis}

\end{tikzpicture}%



==> figures/Aver_Exec_Time/T_av_SCF_2_375.tex <==
\definecolor{MyDarkGreen}{HTML}{006100}
\definecolor{MyBlue}{rgb}{0.00000,0.44700,0.74100}%
\begin{tikzpicture}
  \pgfplotsset{
    label style = {font=\fontsize{9pt}{7.2}\selectfont},
    tick label style = {font=\fontsize{7pt}{7.2}\selectfont}
  }
   \begin{axis}[%
    width=\columnwidth,
    height=\plotfigureheight\columnwidth,
    bar shift auto,
    xmin=0, xmax=17,
    xtick={1,2,...,16},
    xlabel={Maximum number of trials $T_{init}$},
    xlabel style={yshift=0.4em},
    ymin=0.5, ymax=1.5,
    %ytick={0,1,2,...,10},
    ylabel style={yshift=-0.1em},
    ylabel={Average execution time $T_{av}$},
    xlabel style={yshift=-0.2em},
    %ylabel style={yshift=-1.0em},
    % yminorticks, xmajorgrids,
    ymajorgrids, %yminorgrids,
    legend style={legend columns=1},
    legend pos=south east,
    mark size=1.0pt, mark options=solid,
    ]    
    
    \addplot[ybar, bar width=0.5, fill=MyBlue,  draw=black] table[row sep=crcr]{%
      1 1.0\\
      2	1.041672\\
      3	1.072240\\
      4	1.096883\\
      5	1.117481\\
      6	1.135393\\
      7	1.151030\\
      8	1.164988\\
      9 1.177549\\
      10 1.189004\\
      11 1.199519\\
      12 1.209244\\
      13 1.218347\\
      14 1.226894\\
      15 1.234962\\
      16 1.242607\\
      }; 
    
     \addplot[thick, samples=20,line width=1.0pt,  smooth,domain=0:16,red] coordinates {(1,1.15)(16,1.15)};
    
     \addplot[thick, samples=20,line width=1.0pt,  smooth,domain=0:16,MyDarkGreen] coordinates {(1,1.2)(16,1.2)};
    
    \node [](coef1) at (1.8,1.1)
    {\color{red}{\footnotesize{$\upsilon_{pr}=1.15$}}};
    
    \node [](coef2) at (3,1.25)
    {\color{MyDarkGreen}{\footnotesize{$\upsilon_{pr}=1.2$}}};
  
    \end{axis}

    \end{tikzpicture}%

==> figures/FER_SCF/FER_SCF_11_10_var_snr.tex <==
\begin{tikzpicture}
  \pgfplotsset{
    label style = {font=\fontsize{9pt}{7.2}\selectfont},
    tick label style = {font=\fontsize{7pt}{7.2}\selectfont}
  }

  \begin{semilogyaxis}[%
    width=\columnwidth,
    height=\plotfigureheight\columnwidth,
    xtick={1.75,1.875,...,2.5},
    xlabel={$\gamma \left[ \mathrm{dB} \right]$},
    xlabel style={yshift=0.4em},
    ymin=1e-3, ymax=1,
    ylabel style={yshift=-0.1em},
    ylabel={Frame-error rate},
    yminorticks, xmajorgrids,
    ymajorgrids, yminorgrids,
    legend pos=south west,
    mark size=1.0pt, mark options=solid,
    ] 
        
     \addplot[color=red, mark size=2pt, mark=diamond, line width=0.8pt]
    table[row sep=crcr]{%
      1.75	0.2937\\
      1.875	0.2109\\
      2.0	0.1404\\
      2.125	0.0816\\ % 0.08 possible?
      2.25	0.0453\\
      2.375	0.0204\\
      2.5	0.006\\
      };
    \addlegendentry{mechanism} 
    
     \addplot[color=cyan, mark size=2pt, mark=x, line width=0.8pt]
    table[row sep=crcr]{%
      1.75	0.2939\\
      1.875	0.2118\\
      2.0	0.1437\\
      2.125	0.0901\\
      2.25	0.0469\\
      2.375	0.0205\\
      2.5	0.0064\\
      };
    \addlegendentry{balanced} 
       
     \addplot[color=black, mark size=2pt, mark=triangle, line width=0.8pt]
    table[row sep=crcr]{%
      1.75	0.2939\\
      1.875	0.2118\\
      2.0	0.1437\\
      2.125	0.0901\\
      2.25	0.0514\\
      2.375	0.0258\\
      2.5	0.0116\\
      };
    \addlegendentry{sc-mode}    
       
    \addplot[color=blue, mark size=2pt, mark=pentagon, line width=0.8pt]
    table[row sep=crcr]{%
      1.75	0.13\\
      1.875	0.0811\\      
      2.0	0.0478\\      
      2.125	0.0268\\        
      2.25	0.0143\\      
      2.375	0.0073\\
      2.5	0.0035\\
      };
    \addlegendentry{ideal $T_{init}=16$}    
        
  \end{semilogyaxis}

\end{tikzpicture}%

==> figures/FER_SCF/FER_SCF_2_25_var_rate.tex <==
\definecolor{MyDarkGreen}{HTML}{006100}

\begin{tikzpicture}
  \pgfplotsset{
    label style = {font=\fontsize{9pt}{7.2}\selectfont},
    tick label style = {font=\fontsize{7pt}{7.2}\selectfont}
  }

   \begin{semilogyaxis}[%
    width=\columnwidth,
    height=\plotfigureheight\columnwidth,
    xtick=data,
    major x tick style = transparent,
    symbolic x coords={{$1.09$},{$1.11$},{$1.15$},{$1.2$},{$1.25$},{$1.3$},{$1.33$},{$1.4$}},
    xlabel={$\upsilon_{pr}$},
    xlabel style={yshift=0.4em},
    ymin=1e-3, ymax=7e-2,
    %ytick={0,1,2,...,10},
    ylabel style={yshift=-0.1em},
    ylabel={Frame-error rate},
    %ylabel style={yshift=-1.0em},
    yminorticks, xmajorgrids,
    ymajorgrids, yminorgrids,
    legend style={legend columns=2},
    legend pos=south east,
    mark size=1.0pt, mark options=solid,
    ]    

    \addplot[color=red, mark size=2pt, mark=diamond, line width=0.8pt] coordinates{({$1.09$}, 0.047) ({$1.11$}, 0.0431) ({$1.15$}, 0.0374) ({$1.2$}, 0.0312) ({$1.25$}, 0.0263) ({$1.3$}, 0.0224) ({$1.33$}, 0.02) ({$1.4$}, 0.0165)};
    \addlegendentry{\small{multi thr}}      

    \addplot[color=black, mark size=2pt, mark=triangle, line width=0.8pt] coordinates{({$1.09$}, 0.0528) ({$1.11$}, 0.0493) ({$1.15$}, 0.0437) ({$1.2$}, 0.0368) ({$1.25$}, 0.0311)  ({$1.3$}, 0.0264) ({$1.33$}, 0.0227) ({$1.4$}, 0.0171)};
    \addlegendentry{\small{cw drop}} 
    
    \addplot[color=blue, mark size=2pt, mark=x, line width=0.8pt] coordinates{({$1.09$}, 0.0359) ({$1.11$}, 0.0359) ({$1.15$}, 0.0359) ({$1.2$}, 0.0359) ({$1.25$}, 0.0359) ({$1.3$}, 0.0359) ({$1.33$}, 0.0359) ({$1.4$}, 0.0359)};
    \addlegendentry{\small{ideal $T_{init}=4$}}
    
    \addplot[color=MyDarkGreen, mark size=2pt, mark=*, line width=0.8pt] coordinates{({$1.09$}, 0.0215) ({$1.11$}, 0.0215) ({$1.15$}, 0.0215) ({$1.2$}, 0.0215) ({$1.25$}, 0.0215) ({$1.3$}, 0.0215) ({$1.33$}, 0.0215) ({$1.4$}, 0.0215)};
    \addlegendentry{\small{ideal $T_{init}=9$}}    
    
    \addplot[color=yellow, mark size=2pt, mark=pentagon, line width=0.8pt] coordinates{({$1.09$}, 0.0143) ({$1.11$}, 0.0143) ({$1.15$}, 0.0143) ({$1.2$}, 0.0143) ({$1.25$}, 0.0143) ({$1.3$}, 0.0143) ({$1.33$}, 0.0143) ({$1.4$}, 0.0143)};
    \addlegendentry{\small{ideal $T_{init}=16$}}   
    
 
  \end{semilogyaxis}

\end{tikzpicture}%

==> figures/FER_SCF/FER_SCF_2_375_var_rate.tex <==
\definecolor{MyDarkGreen}{HTML}{006100}

\begin{tikzpicture}
  \pgfplotsset{
    label style = {font=\fontsize{9pt}{7.2}\selectfont},
    tick label style = {font=\fontsize{7pt}{7.2}\selectfont}
  }

   \begin{semilogyaxis}[%
    width=\columnwidth,
    height=\plotfigureheight\columnwidth,
    xtick=data,
    major x tick style = transparent,
    symbolic x coords={{$1.0667$},{$1.0909$},{$1.11$},{$1.1429$},{$1.15$},{$1.1667$},{$1.2$},{$1.25$}},
    xlabel={$\upsilon_{pr}$},
    xlabel style={yshift=0.4em},
    ymin=1e-3, ymax=5e-2,
    %ytick={0,1,2,...,10},
    ylabel style={yshift=-0.1em},
    ylabel={Frame-error rate},
    %ylabel style={yshift=-1.0em},
    yminorticks, xmajorgrids,
    ymajorgrids, yminorgrids,
    legend style={legend columns=2},
    legend pos=south east,
    mark size=1.0pt, mark options=solid,
    ]    

    \addplot[color=red, mark size=2pt, mark=diamond, line width=0.8pt] coordinates{({$1.0667$}, 0.0259) ({$1.0909$}, 0.0217) ({$1.11$}, 0.0189) ({$1.1429$}, 0.0151) ({$1.15$}, 0.0146) ({$1.1667$}, 0.0128) ({$1.2$}, 0.0103) ({$1.25$}, 0.0078)};
    \addlegendentry{\small{multi thr.}} 
    
     \addplot[color=black, mark size=2pt, mark=triangle, line width=0.8pt] coordinates{({$1.0667$}, 0.0301) ({$1.0909$}, 0.026) ({$1.11$}, 0.0228) ({$1.1429$}, 0.0184) ({$1.15$}, 0.0176) ({$1.1667$}, 0.0154) ({$1.2$}, 0.0117) ({$1.25$}, 0.0078)};
    \addlegendentry{\small{cw drop.}}     
    
    \addplot[color=magenta, mark size=2pt, mark=|, line width=0.8pt] coordinates{({$1.0667$}, 0.0246) ({$1.0909$}, 0.0246) ({$1.11$}, 0.0246) ({$1.1429$}, 0.0246) ({$1.15$}, 0.0246)  ({$1.1667$}, 0.0246) ({$1.2$}, 0.0246) ({$1.25$}, 0.0246)};
    \addlegendentry{\small{ideal $T_{init}=3$}}
    
    \addplot[color=blue, mark size=2pt, mark=x, line width=0.8pt] coordinates{({$1.0667$}, 0.0140) ({$1.0909$}, 0.0140) ({$1.11$}, 0.0140) ({$1.1429$}, 0.0140) ({$1.15$}, 0.0140)  ({$1.1667$}, 0.0140) ({$1.2$}, 0.0140) ({$1.25$}, 0.014)};
    \addlegendentry{\small{ideal $T_{init}=7$}}
    
    \addplot[color=MyDarkGreen, mark size=2pt, mark=*, line width=0.8pt] coordinates{({$1.0667$}, 0.0105) ({$1.0909$}, 0.0105) ({$1.11$}, 0.0105) ({$1.1429$}, 0.0105) ({$1.15$}, 0.0105)  ({$1.1667$}, 0.0105) ({$1.2$}, 0.0105) ({$1.25$}, 0.0105)};
    \addlegendentry{\small{ideal $T_{init}=10$}}    
    
    \addplot[color=yellow, mark size=2pt, mark=pentagon, line width=0.8pt] coordinates{({$1.0667$}, 0.0073) ({$1.0909$}, 0.0073) ({$1.11$}, 0.0073) ({$1.1429$}, 0.0073) ({$1.15$}, 0.0073)  ({$1.1667$}, 0.0073) ({$1.2$}, 0.0073) ({$1.25$}, 0.0073)};
    \addlegendentry{\small{ideal $T_{init}=16$}}
    
  \end{semilogyaxis}

\end{tikzpicture}%

==> figures/FER_SCF/FER_SCF_6_5_var_snr.tex <==
\begin{tikzpicture}
  \pgfplotsset{
    label style = {font=\fontsize{9pt}{7.2}\selectfont},
    tick label style = {font=\fontsize{7pt}{7.2}\selectfont}
  }

  \begin{semilogyaxis}[%
    width=\columnwidth,
    height=\plotfigureheight\columnwidth,
    xtick={1.75,1.875,...,2.5},
    xlabel={$\gamma \left[ \mathrm{dB} \right]$},
    xlabel style={yshift=0.4em},
    ymin=1e-3, ymax=1,
    ylabel style={yshift=-0.1em},
    ylabel={Frame-error rate},
    yminorticks, xmajorgrids,
    ymajorgrids, yminorgrids,
    legend pos=south west,
    mark size=1.0pt, mark options=solid,
    ]       
    
     \addplot[color=red, mark size=2pt, mark=x, line width=0.8pt]
    table[row sep=crcr]{%
      1.75	0.2803\\
      1.875	0.1882\\
      2.0	0.119\\
      2.125	0.0666\\
      2.25	0.0312\\
      2.375	0.0103\\
      2.5	0.0035\\
      };
    \addlegendentry{multi thr.}    
    
    \addplot[color=black, mark size=2pt, mark=triangle, line width=0.8pt]
    table[row sep=crcr]{%
      1.75	0.2847\\
      1.875	0.1991\\
      2.0	0.1287\\
      2.125	0.0749\\
      2.25	0.0368\\
      2.375	0.0117\\
      2.5	0.0035\\
      };
    \addlegendentry{cw drop.}        
       
    \addplot[color=blue, mark size=2pt, mark=pentagon, line width=0.8pt]
    table[row sep=crcr]{%
      1.75	0.13\\
      1.875	0.0811\\      
      2.0	0.0478\\      
      2.125	0.0268\\        
      2.25	0.0143\\      
      2.375	0.0073\\
      2.5	0.0035\\
      };
    \addlegendentry{ideal}    
        
  \end{semilogyaxis}

\end{tikzpicture}%
